Spatial Relation Graph and Graph Convolutional Network for Object Goal Navigation

This paper describes a framework for the object-goal navigation task, which requires a robot to find and move to the closest instance of a target object class from a random starting position. The framework uses a history of robot trajectories to learn a Spatial Relational Graph (SRG) and Graph Convolutional Network (GCN)-based embeddings for the likelihood of proximity of different semantically-labeled regions and the occurrence of different object classes in these regions. To locate a target object instance during evaluation, the robot uses Bayesian inference and the SRG to estimate the visible regions, and uses the learned GCN embeddings to rank visible regions and select the region to explore next.

==> 2_problem.tex <==
\section{Problem Definition}\label{sec:prob}
The paper addresses the problem of \textit{ObjectNav} \cite{batra2020objectnav} in which an agent is initialized at a random pose in an unknown indoor environment and is asked to find the nearest goal object instance by exploration. At every step, the agent has to choose the next action \textit{a} $\in$  \textit{A}, from set of actions \textit{A} = \{\textit{`Stop'}, \textit{`Move\_Forward'}, \textit{`Turn\_Left'}, \textit{`Turn\_Right'}, \textit{`Look\_Up'}, \textit{`Look\_Down'}\}. An episode is considered a `success', if the  agent is within $1.0$ metre Euclidean distance from any instance of the target object (goal).

\Madhav{As discussed Problem Definition need not be from Habitat internals perspective. The agent needing to choose one of the 4 actions is a Habitat abstraction and not the way the problem is solved. You should mention what is the problem actually being solved. But this should come after related work along with the pipeline. You pose the problem, show the pipeline image and quickly delineate the solution}



==> 5.1_experimental_setup.tex <==
\subsection{\textbf{\textit{Experimental Setup :}}}

The house scene data from Matterport3d (MP3D) \cite{Matterport3D} is used as benchmark in AI Habitat simulator. It includes semantic annotations of regions like `bathroom', `bedroom', etc. We generate the spatial-common sense graph from $59$ scenes of MP3D dataset. For each scene,  we initialize the agent at region $R_i$ and allow the agent to traverse to all other regions  present in scenes using the simulator. We obtain a scene graph for every house/scene of MP3D data.
Two region nodes $n_{R_k}$ and $n_{R_l}$ are connected in a graph if regions $R_k$ and $R_l$ are adjacent in the scene and there exists a direct path which an agent can traverse with no intermediate regions. For instance, if \textit{garage} and \textit{bedroom} are adjacent in a scene but to reach \textit{garage} starting from \textit{bedroom}, an agent has to traverse \textit{hallway} and \textit{entryway}, then there will be no edge connecting the nodes representing regions \textit{garage} and \textit{bedroom}. Also, for each region, we connect the objects present in region with the node corresponding to that region. From the $59$ scene graphs, we construct the spatial relational graph using the approach mentioned in Section~\ref{section:common_sense_graph_generation}. We use NetworkX ~\cite{hagberg2008exploring}, a Python package for graph creation, manipulation and implementation to represent the spatial information present in \textit{MP3D} scenes.

We train the GCN on $12$ \textit{MP3D} scenes and we evaluate our approach
on 1500 episodes ($6$ \textit{Matterport3d} scenes, 250 episodes for each scene). We use 3-layer GCN which takes 
    i) Spatial relational graph as input graph and  
    ii) one  hot  encoding  vector  of  region  and  object  nodes as input feature. 
$18,488$  valid trajectories obtained using approach mentioned in Section~\ref{section:trajectory_path_generation} are used to train the GCN. Sigmoid Cross-Entropy loss is used to learn embeddings for region and object nodes. While training, we use Adam optimizer with a learning rate of 0.0003 to update network weights iteratively based on trajectory data. We use GCNConv operator for the $3$ convolutional layers. The reason for choosing GCNConv~\cite{kipf2016semi} is that it learns hidden layer representations that encode both local graph structure and features of nodes. Also, it scales linearly with increase in edges in the graph. We assume the agent knows the entire map, the objects and regions present in the scene. For each scene, we allow the agent to traverse from region $R_{i}$ to all other regions $R_j$ ($i$, $j$ $\in$  {$R_{1}$, $R_{2}$, $R_{3}$,..., $R_{n}$} , $i$$\neq$$j$). For each scene, we create an edge between two region nodes if two regions are adjacent in the path that exists between $R_{i}$  and $R_{j}$ . Also, we create an edge between object node ($n_{o}$) and region node ($n_{R_i}$) if the object o is present in region $R_{i}$. We create such \textit{scene graphs} ($G_{1}$, $G_{2}$, $G_{3}$,  ......., $G_{59}$ $\in$ $G$) for $59$ scenes in the MP3D data. The final $G_{s}$ after processing as per section \ref{section:common_sense_graph_generation} consists of $47$ nodes and $104$ edges. We use PyTorch Geometric ~\cite{fey2019fast} which is a deep learning library for PyTorch to work with GCN. Figure~\ref{fig:trajectory_video} depicts the path traversed by agent in scene \textit{b8cTxDM8gDG} of MP3D dataset to reach the target object \textit{i.e.} bathtub starting from the  kitchen. Agent travels through the regions kitchen(a) $\rightarrow$ hallway (b) $\rightarrow$ bedroom (c) $\rightarrow$ bathroom (e) $\rightarrow$ bathtub (f) at increasing timesteps.

==> 5.2_baselines.tex <==
\subsection{\textbf{\textit{Comparison with Baselines :}}}

Following common practice, object categories (like window, door, passage) other than the selected 19 types are eliminated because they are not the de-facto objects to find. For $6$ MP3D scenes \{17DRP5sb8fy, rPc6DW4iMge, S9hNv5qa7GM, b8cTxDM8gDG, EDJbREhghzL, 2azQ1b91cZZ\} and $19$ object categories, we evaluate the performance of our approach via the same metrics used earlier: Success, SPL and DTS. The quantitative results of Object Navigation using our approach compared with the baselines are shown in Table \ref{table:comparison_with_baselines}. In the random based exploration, the agent randomly chooses any random action from the set of motion actions. The agent stops when the episode gets over i.e when maximum number of permitted steps are achieved or the target is found. Frontier Based Exploration~\cite{yamauchi1997frontier} allows the agent to move to the boundary between open space and unexplored territory. If the target object is visible, it moves towards that and issues a STOP action. Else, the agent moves towards the successive frontiers , thereby constantly gaining information about the world. In contrast to Frontier based exploration, in Active Neural Slam (ANS) approach~\cite{chaplot2020learning}, the agent moves towards the target object with the goal to maximize the coverage in fixed time. Coverage is defined as a traversable area in the map. As depicted in Table \ref{table:comparison_with_baselines}, the \textit{semNav} outperforms the standard baselines by significant margin. For experiments, we assume that the region associated with the visible object is known. We compute the \textit{walk score} based on the node embeddings of last node in history of traversed regions, the visible regions and target object. The agent moves towards the visible region having \textit{maximum} walk score.

We also evaluate on 6 object categories (‘chair’, ‘couch’, ‘plant’, ‘bed’, ‘toilet’ and ‘tv’) with the latest state of art SemExp \cite{chaplot2020object} on MP3D dataset. It is found that performance on this object categories is better than the baselines run on all categories. One possible reason is that these 6 objects has very close attachment to their regions, whereas say an object category namely `picture' can be located at multiple locations. Apart from these object detection algorithms also plays a role in success. As an example, `shower' category is difficult to detect due to its position inside a bathroom. Also, it's bounding box comprises sparse area and may cover other objects like `towel'.

==> 5.3_ablation_analysis.tex <==

\subsection{\textbf{\textit{Ablation Study :}}}
To understand the contribution of the spatial relation statistics and valid trajectory data for GCN training in \textit{semNav}, we perform some ablation studies. For individual specific goal categories, we find the performance of navigating and finding the object with and without training the GCN using spatial relational graph and trajectory  data. In this, we allowed the agent to move towards any random visible object in contrast to our approach. In our approach, the agent moves towards the object present in the region that corresponds to maximum walk score. The ablation study analyzes the effect of bias caused by embeddings generated by training the GCN on `train' set. We replace the score function with the random function and agent moves towards any random object chosen from the set of visible objects. The performance of \textit{semNav} approach without using the spatial relations and trajectory data declines as depicted in Table \ref{table:ablation_table}.

The spatial graph has been constructed while taking 59 scenes of MP3D data into consideration. The spatial graph is generalized and not biased towards a particular scene or walk. At the navigation run-time, we evaluate the performance of our approach on $6$ scenes and the results in Table \ref{table:ablation_table} showcase the inference from specific scenes on particular target object search.
\begin{table}
\caption{\textbf{Ablation Analysis} : Comparison of  performance of \textit{semNav} on $19$ objects on $6$ scenes with and without using spatial relations and trajectory data during GCN training.}
\centering
\hline
\begin{tabular}{| *{5}{c|} }
Target Object & \multicolumn{2}{c|}{Without Spatial Relation} & \multicolumn{2}{c|}{\textbf{With Spatial Relation}} \\
 & Success $\uparrow$  &  SPL $\uparrow$ & Success $\uparrow$  &  SPL $\uparrow$ \\
\hline
bed & 0.60 &  0.3484 & 0.9983 &  0.678 \\
towel & 0.4366 & 0.2075 & 0.8666 & 0.5258 \\
chair & 0.88 & 0.615  & 0.9383 & 0.696 \\
shower & 0.63 & 0.2761 & 0.875 & 0.521 \\
picture & 0.395  & 0.3576 & 0.95 & 0.7321
\label{table:ablation_table}
\end{tabular}
\hline
\end{table}

==> supplimentary_material.tex <==
\cleardoublepage

\begin{table*}[t]
\caption{19 target objects - 6 scenes -spatial relational graph .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 97.2\% & 93.2\% & 90.4\% & 95.199\% & 96.8\% & 92.0\% & 94.133\%\\
SPL & 0.71217 & 0.63095203 & 0.62110938 & 0.725328 & 0.68575 & 0.5738964 & 0.658\%\\
SoftSPL & 0.72713 & 0.644370 & 0.6442022 & 0.74555085 & 0.71081 & 0.6039638 & 0.67931\\
DTS & 0.01170 & 0.45190313 & 0.6674027 & 0.29111623 & 0.05681 & 0.3497 & 0.3047\\
\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{target object- BED - 6 scenes - random object .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 98.0-98.0\% & 82.0-82.0\% & 22.0-22.0\% & 28.0-28.0000\% & 40.0-40.0\% & 90.0-90.0\% & 60\%\\
SPL & 0.7874150 & 0.3127048 & 0.11991 & 0.2192129 & 0.12750 & 0.52414652 & 0.3484\\

\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{target object- BED - 6 scenes - spatial relation graph.}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 100.0-100.0\% & 99.0-99.0\% & 100.0-100.0\% & 100-100\% & 100-100\% & 100-100\% & 99.83\\
SPL & 0.8838 & 0.5607001 & 0.60738379  & 0.803218 & 0.529856627 & 0.6842170 & 0.67803\\

\hline
\end{tabular}
\end{table*}




\begin{table*}[t]
\caption{target object- TOWEL - 6 scenes - random object .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 99.0-99.0\% & 2.0-2.0\% & 61.0-61.0\% & 41.0-41.0\% & 57.0-56.999\% & 2.0-2.0\% & 43.66\%\\
SPL & 0.544416 & 0.014903 & 0.2072007 & 0.21482 & 0.26191 & 0.0034244455 & 0.2075\\

\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{target object- TOWEL - 6 scenes - spatial relational graph .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & 86.66\%\\
\hline
Success & 100.0-100.0\% & 58.0-57.99\% & 96.0-96.0\% & 95.0-95.0\% & 88.0-88.0\% & 83.0-83.0\% & 86.66\%\\
SPL & 0.7289 & 0.4545 & 0.52725  & 0.359044 & 0.60414 & 0.48103 & 0.5258\\

\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{target object- CHAIR - 6 scenes - random object .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 98.0-98.0\% & 97.0-97.0\% & 55.0-55.000\% & 92.0-92.0\% & 97.0-97.0\% & 89.0-89.0\% & 88\%\\
SPL & 0.7487202383503 & 0.630283 & 0.20917 & 0.727183 & 0.88803 & 0.4916503 & 0.615\\

\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{target object- CHAIR - 6 scenes - spatial relational graph .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 99.0-99.0\% & 100.0-100.0\% & 73.0-73.0\% & 100-100\% & 97-97\% & 94-94\% & 93.83\%\\
SPL & 0.803899 & 0.684538 & 0.499564343  & 0.860181 & 0.8696 & 0.462590 & 0.696\\

\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{target object- SHOWER - 6 scenes - random object .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 73.0-73.0\% & 79.0-79.0\% & 44.0-44.0\% & 58.0-57.999\% & 62.0-62.0\% & 62.0-62.0\% & 63\%\\
SPL & 0.24856 & 0.262345 & 0.18526717 & 0.46956 & 0.3318 & 0.15955 & 0.2761\\

\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{target object- SHOWER - 6 scenes - spatial relational graph .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 93.0-93.0\% & 81.0-81.0\% & 68.0-68.0\% & 93.0-93.0\% & 90.0-90.0\% & 100.0-100.0\% & 87.5\%\\
SPL & 0.564670147 & 0.3739251 & 0.34659  & 0.684873 & 0.55484 & 0.603816768 & 0.521\\

\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{target object- PICTURE - 6 scenes - random object .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 37.0-37.0\% & 45.0-45.0\% & 17.0-17.0\% & 71.0-71.0\% & 58.0-57.999\% & 9.0-9.0\% & 39.5\%\\
SPL & 0.3671 & 0.40025 & 0.1290 & 0.6759 & 0.51302 & 0.060869 & 0.3576\\

\hline
\end{tabular}
\end{table*}


\begin{table*}[t]
\caption{target object- PICTURE - 6 scenes - spatial relational graph .}
\centering
\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\hline
Scene & 17DRP5sb8fy & rPc6DW4iMge & S9hNv5qa7GM & b8cTxDM8gDG & EDJbREhghzL & 2azQ1b91cZZ & Average\\
\hline
Success & 100.0-100.0\% & 99.0-99.0\% & 86.0-86.0\% & 95.0-95.0\% & 100-100\% & 90-90\% & 95\%\\
SPL & 0.9585802 & 0.7968499 & 0.64060811  & 0.77609 & 0.75929 & 0.4618838 & 0.7321\\

\hline
\end{tabular}
\end{table*}







